Palette Sparsification Beyond $(\Delta+1)$ Vertex Coloring

A recent palette sparsification theorem of Assadi, Chen, and Khanna [SODA'19] states that in every $n$-vertex graph $G$ with maximum degree $\Delta$, sampling $O(\log{n})$ colors per each vertex independently from $\Delta+1$ colors almost certainly allows for proper coloring of $G$ from the sampled colors. Besides being a combinatorial statement of its own independent interest, this theorem was shown to have various applications to design of algorithms for $(\Delta+1)$ coloring in different models of computation on massive graphs such as streaming or sublinear-time algorithms. In this paper, we further study palette sparsification problems: * We prove that for $(1+\varepsilon) \Delta$ coloring, sampling only $O_{\varepsilon}(\sqrt{\log{n}})$ colors per vertex is sufficient and necessary to obtain a proper coloring from the sampled colors. * A natural family of graphs with chromatic number much smaller than $(\Delta+1)$ are triangle-free graphs which are $O(\frac{\Delta}{\ln{\Delta}})$ colorable. We prove that sampling $O(\Delta^{\gamma} + \sqrt{\log{n}})$ colors per vertex is sufficient and necessary to obtain a proper $O_{\gamma}(\frac{\Delta}{\ln{\Delta}})$ coloring of triangle-free graphs. * We show that sampling $O_{\varepsilon}(\log{n})$ colors per vertex is sufficient for proper coloring of any graph with high probability whenever each vertex is sampling from a list of $(1+\varepsilon) \cdot deg(v)$ arbitrary colors, or even only $deg(v)+1$ colors when the lists are the sets $\{1,\ldots,deg(v)+1\}$. Similar to previous work, our new palette sparsification results naturally lead to a host of new and/or improved algorithms for vertex coloring in different models including streaming and sublinear-time algorithms.

==> app-prelim.tex <==
% !TeX root = main.tex 
%!TEX root = main.tex


\section{Probabilistic Tools}\label{sec:prob}

We use the following standard probabilistic tools. 

\begin{proposition}[Lov\'asz Local Lemma -- symmetric form; 
cf.~\cite{ProbBook}]\label{prop:lll}
	 Let $\event_1,\ldots,\event_n$ be $n$ events such that 
each event $\event_i$ is mutually independent of all other events 
besides at most $d$, and $\Pr\paren{\event_i} \leq p$ for all $i \in [n]$. If $e \cdot p \cdot (d+1) \leq 1$ (where $e=2.71...$), then $\Pr\paren{\wedge_{i=1}^{n} \overline{\event_i}} > 0$. 
\end{proposition}


\begin{proposition}[Chernoff-Hoeffding bound; cf.~\cite{ProbBook}]\label{prop:chernoff}
	Let $X_1,\ldots,X_n$ be $n$ independent random variables where each $X_i \in [0,b]$. Define $X:= \sum_{i=1}^{n} X_i$. Then, for any $t > 0$, 
	\begin{align*}
		\Pr\Paren{\card{X - \expect{X}} > t} \leq 2 \cdot \exp\paren{-\frac{2t^2}{n \cdot b^2}}.
	\end{align*}
	Moreover, for any $\delta \in (0,1)$, 
	\begin{align*}
		\Pr\Paren{\card{X - \expect{X}} > \delta \cdot \expect{X}} \leq 2 \cdot \exp\paren{-\frac{\delta^2 \cdot \expect{X}}{3b}}.
	\end{align*} 
\end{proposition}

A function $f(x_1,\ldots,x_n)$ is called \emph{$c$-Lipschitz} iff changing any single $x_i$ can affect the value of $f$ by at most $c$. Additionally, $f$ is called \emph{$r$-certifiable} iff whenever $f(x_1,\ldots,x_n) \geq s$, there exists
at most $r \cdot s$ variables $x_{i_1},\ldots,x_{i_{r \cdot s}}$ so that knowing the values of these variables certifies $f \geq s$. 


\begin{proposition}[Talagrand's inequality; cf.~\cite{ColoringBook}]\label{prop:talagrand}
	Let $X_1,\ldots,X_n$ be $n$ independent random variables and $f(X_1,\ldots,X_n)$ be a $c$-Lipschitz function; then for any $t \geq 1$, 
	\begin{align*}
		\Pr\paren{\card{f - \expect{f}} > t } \leq 2 \exp\paren{-\frac{t^2}{2c^2 \cdot n}}.
	\end{align*} 
	 Moreover, if $f$ is additionally $r$-certifiable, then for any $b \geq 1$,
	\begin{align*}
		\Pr\paren{\card{f - \expect{f}} > b + 30c \sqrt{r \cdot \expect{f}}} \leq 4 \exp\paren{-\frac{b^2}{8c^2 r \expect{f}}}. 
	\end{align*} 
\end{proposition}



==> other-sublinear.tex <==
% !TeX root = main.tex 
%!TEX root = main.tex

\section{Applications to Other Models of Computation \TAG}\label{app:other-sublinear}

\subsection{Massively Parallel Computation Model}\label{sec:mpc}

\begin{remark}[Distributed Sketching Model]
\end{remark}

\subsection{Congested Clique Model}\label{sec:congest}

\subsection{Dynamic Graph Algorithms}\label{sec:dynamic}

%%\subsection{Distributed Sketching Model}\label{sec:sketching}
